CoinSeg: Contrast Inter- and Intra- Class Representations for Incremental Segmentation

Class incremental semantic segmentation aims to strike a balance between the model's stability and plasticity by maintaining old knowledge while adapting to new concepts. However, most state-of-the-art methods use the freeze strategy for stability, which compromises the model's plasticity.In contrast, releasing parameter training for plasticity could lead to the best performance for all categories, but this requires discriminative feature representation.Therefore, we prioritize the model's plasticity and propose the Contrast inter- and intra-class representations for Incremental Segmentation (CoinSeg), which pursues discriminative representations for flexible parameter tuning. Inspired by the Gaussian mixture model that samples from a mixture of Gaussian distributions, CoinSeg emphasizes intra-class diversity with multiple contrastive representation centroids. Specifically, we use mask proposals to identify regions with strong objectness that are likely to be diverse instances/centroids of a category. These mask proposals are then used for contrastive representations to reinforce intra-class diversity. Meanwhile, to avoid bias from intra-class diversity, we also apply category-level pseudo-labels to enhance category-level consistency and inter-category diversity. Additionally, CoinSeg ensures the model's stability and alleviates forgetting through a specific flexible tuning strategy. We validate CoinSeg on Pascal VOC 2012 and ADE20K datasets with multiple incremental scenarios and achieve superior results compared to previous state-of-the-art methods, especially in more challenging and realistic long-term scenarios. Code is available at https://github.com/zkzhang98/CoinSeg.

==> a_figures/quat_ade.tex <==
\begin{figure*}[t]
\centering 
{\includegraphics[width=1.00\linewidth]{materials/quat_ade.pdf}
}
\vspace{-8mm}
\caption{{Qualitative analysis for ADE 100-10.}}
% \vspace{-0.3cm}
\label{fig:quat_ade}
 \end{figure*}

==> a_figures/quat_more.tex <==
\begin{figure*}[t]
\centering 

{\includegraphics[width=0.95\linewidth]{materials/supp_quat_voc.pdf}
}

\caption{{More qualitative analysis of CoinSeg. The white borderline is \textbf{ignore label} in Pascal VOC 2012 dataset.}}
% \vspace{-0.3cm}
\label{fig:quat_more}
 \end{figure*}

==> a_figures/quat_more2.tex <==
\begin{figure*}[t]
\centering 

{\includegraphics[width=0.95\linewidth]{materials/supp_quat_voc_2.pdf}
}

\caption{{More qualitative analysis of CoinSeg. The white borderline is \textbf{ignore label} in Pascal VOC 2012 dataset.}}
% \vspace{-0.3cm}
\label{fig:quat_more2}
 \end{figure*}

==> a_tables/A_corrected.tex <==
\begin{table*}[t!]
  \centering
\caption{
    Corrected Tab.1 in main paper. The correct values are highlighted in \textcolor{red}{red}. 
  }
  \label{tab:corrected}
  \begin{adjustbox}{max width=\linewidth}
  \begin{tabular}{l|c|ccc|ccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multicolumn{3}{c|}{\textbf{VOC 10-1 (11 steps)}} & \multicolumn{3}{c|}{\textbf{VOC 15-1 (6 steps)}} & \multicolumn{3}{c|}{\textbf{VOC 19-1 (2 steps)}} & \multicolumn{3}{c|}{\textbf{VOC 15-5 (2 steps)}} & \multicolumn{3}{c}{\textbf{VOC 2-2 (10 steps)}} \\
 &  & 0-10 & 11-20 & all & 0-15 & 16-20 & all & 0-19 & 20 & all & 0-15 & 16-20 & all & 0-2 & 3-20 & all \\ \midrule
\textcolor{lightgray}{Joint} & \textcolor{lightgray}{ResNet101} & \textcolor{lightgray}{82.1}  & \textcolor{lightgray}{79.6} & \textcolor{lightgray}{80.9} & \textcolor{lightgray}{82.7} & \textcolor{lightgray}{75.0} & \textcolor{lightgray}{80.9} & \textcolor{lightgray}{81.0} & \textcolor{lightgray}{79.1} & \textcolor{lightgray}{80.9} & \textcolor{lightgray}{82.7} & \textcolor{lightgray}{75.0} & \textcolor{lightgray}{80.9} & \textcolor{lightgray}{76.5} & \textcolor{lightgray}{81.6} & \textcolor{lightgray}{80.9} \\
LwF-MC~\cite{LwF_li2017learning} & ResNet101 & 4.7 & 5.9 & 4.9 & 6.4 & 8.4 & 6.9 & 64.4 & 13.3 & 61.9 & 58.1 & 35.0 & 52.3 & 3.5 & 4.7 & 4.5\\
ILT~\cite{ILT_michieli2019incremental} & ResNet101 & 7.2 & 3.7 & 5.5 & 8.8 & 8.0 & 8.6 & 67.8 & 10.9 & 65.1 & 67.1 & 39.2 & 60.5 & 5.8 & 5.0 & 5.1 \\
MiB~\cite{MiB} & ResNet101 & 12.3 & 13.1 & 12.7 & 34.2 & 13.5 & 29.3 & 71.4 & 23.6 & 69.2 & 76.4 & 50.0 & 70.1 & 41.1 & 23.4 & 25.9 \\
SDR~\cite{SDR} & ResNet101 & 32.1 & 17.0 & 24.9 & 44.7 & 21.8 & 39.2 & 69.1 & 32.6 & 67.4 & 57.4 & 52.6 & 69.9 & 13.0 & 5.1 & 6.2 \\
PLOP~\cite{PLOP} & ResNet101 & 44.0 & 15.5 & 30.5 & 65.1 & 21.1 & 54.6 & 75.4 & 37.4 & 73.5 & 75.7 & 51.7 & 70.1 & 24.1 & 11.9 & 13.7 \\
RCIL~\cite{RCIL} & ResNet101 & 55.4 & 15.1 & 34.3 & 70.6 & 23.7 & 59.4 & 68.5 & 12.1 & 65.8 & 78.8 & 52.0 & 72.4 & 28.3 & 19.0 & 19.4 \\
SSUL~\cite{SSUL} & ResNet101 & 71.3 & 46.0 & 59.3 & 77.3 & 36.6 & 67.6 & 77.7 & 29.7 & 75.4 & 77.8 & 50.1 & 71.2 & 62.4 & 42.5 & 45.3 \\

MicroSeg~\cite{MicroSeg} & ResNet101 & 72.6 & 48.7 & 61.2 & 80.1 & 36.8 & 69.8 & 78.8 & 14.0 & 75.7 & 80.4 & 52.8 & 73.8 & 61.4 & 40.6 & 43.5 \\

\midrule
\textcolor{lightgray}{Joint\dag} & \textcolor{lightgray}{Swin-B} & \textcolor{lightgray}{82.4} & \textcolor{lightgray}{83.0} & \textcolor{lightgray}{82.7} & \textcolor{lightgray}{83.8} & \textcolor{lightgray}{79.3} & \textcolor{lightgray}{82.7} & \textcolor{lightgray}{82.6} & \textcolor{lightgray}{84.4} & \textcolor{lightgray}{82.7} & \textcolor{lightgray}{83.8} & \textcolor{lightgray}{79.3} & \textcolor{lightgray}{82.7} & \textcolor{lightgray}{75.8} & \textcolor{lightgray}{83.9} & \textcolor{lightgray}{82.7} \\
SSUL\dag\cite{SSUL} & Swin-B & 74.3 & 51.0 & 63.2 & 78.1 & 33.4 & 67.5 & 80.8 & 31.5 & 78.4 & 79.7 & 55.3 & 73.9 & 60.3 & 40.6 & 44.0 \\

MicroSeg\dag~\cite{MicroSeg} & Swin-B & 73.5 & 53.0 & 63.8 & 80.5 & 40.8 & 71.0 & 79.0 & 25.3 & 76.4 & \textcolor{red}{81.9} & \textcolor{red}{54.0} & \textcolor{red}{75.2} & 64.8 & 43.4 & 46.5 \\

\midrule
\methodname~(Ours) & Swin-B & \textbf{80.0} & \textbf{63.4} & \textbf{72.5} & \textbf{82.7} & \textbf{52.5} & \textbf{75.5} & \textbf{81.5} & \textbf{44.8} & \textbf{79.8} & \textbf{82.1} & \textbf{63.2} & \textbf{77.6} & \textbf{70.1} & \textbf{63.3} & \textbf{64.3} \\ 

\bottomrule
\end{tabular}
  \end{adjustbox}
\end{table*}




==> a_tables/MicroSeg_choice_of_K.tex <==
\begin{table}[h]
\color[rgb]{0,0,0.18} 
    \vspace{-2mm}
  \centering
  \caption{
     Hyperparameter search of $K$ in MicroSeg with Swin-B backbone (Left), and $\lambda_c$ within a similar magnitude~(Right).
  }
  \label{tab:choiceOfK}
  \begin{adjustbox}{max width=0.96\linewidth}
     \begin{tabular}{c|ccc}
\toprule
\multirow{2}{*}{$K$} & \multicolumn{3}{c}{VOC 15-1 (6 steps)} \\
 & 0-15 & 16-20 & all \\ 
 \midrule
1 & 78.8 & 37.1 & 68.9 \\
3 & 79.1 & 38.6 & 69.5 \\
5 & 80.5 & 40.8 & \textbf{71.0} \\
7 & 81.4 & 35.9 & 70.6 \\
9 & 81.2 & 36.1 & 70.4 \\ 
\bottomrule
\end{tabular}
  
  \end{adjustbox}
  \vspace{-6mm}
\end{table}

==> a_tables/PL_Lint.tex <==
\begin{table}[h]
\centering
  \vspace{-2mm}
  \caption{
  % \textcolor[rgb]{0.01,0.01,0.15}{
     Ablations to pseudo-labeling  in $\mathcal{L}_{int}$. 
     GT: ground truth, PL: pseudo label.
  }
  \label{tab:PL_Lint}
  \begin{adjustbox}{max width=0.96\linewidth}
     \begin{tabular}{c|ccc}
      \toprule
    \multirow{2}{*}{label}     &\multicolumn{3}{c}{\textbf{VOC 15-1 (6 steps)}}      \\
 &   0-15          & 16-20         & all                \\ \midrule
              
 GT & 81.6  & 54.3   & 75.1        \\
                                                            
 PL & 82.7 & 52.5 & \textbf{75.5} \\

      \bottomrule
    \end{tabular}
  
  \end{adjustbox}
  \vspace{-2mm}
\end{table}

==> a_tables/abl_con.tex <==
\begin{table}[t]
  \centering
  \caption{
     Parameter search of hyper-parameter to balance \textit{Coin}, $\lambda_c$. All experiments are conducted on VOC 15-1.
}
  \label{tab:abl_con}
  \begin{adjustbox}{max width=\linewidth}
     \begin{tabular}{cc|ccc}
      \toprule
      \multirow{2}{*}{{Method}}  &\multirow{2}{*}{$\lambda_c$} & \multicolumn{3}{c}{\textbf{VOC 15-1 (6 steps)}}                                                                  \\
                          &                                       & 0-15          & 16-20         & all                   \\ \midrule
       \multirow{5}{*}{CoinSeg}                             
                        & $10^{-3}$ & 81.4          & 48.9          & 73.7                  \\
                        & $0.01$ & 82.7          & 52.5          & \textbf{75.5}          \\
                        & $0.1$ & 82.4          & 51.8          & 75.1          \\
                        & $1$ & 81.8 & 49.9 & 74.2 \\
                        & $10$ & 80.6 & 46.6 & 72.5 \\
      \bottomrule
    \end{tabular}
  
  \end{adjustbox}
  \vspace{-2mm}
\end{table}

==> a_tables/abl_intra.tex <==
\begin{table}[t]
  \centering
  \caption{
     Ablation study of Contrast inter- \& intra- class representations, $\lambda_r$. All experiments are conducted on VOC 15-1.
  }
  \label{tab:abl_intra}
  \begin{adjustbox}{max width=\linewidth}
     \begin{tabular}{ccc|ccc}
      \toprule
      \multirow{2}{*}{{Method}} & \multirow{2}{*}{$\mathcal{L}_{int}$} &\multirow{2}{*}{$\mathcal{L}_{itr}$} & \multicolumn{3}{c}{\textbf{VOC 15-1 (6 steps)}}                                                                  \\
                          &                                     &  & 0-15          & 16-20         & all                   \\ \midrule
       \multirow{3}{*}{CoinSeg}                
                      & \xmark                                      & \xmark & 80.4  & 43.7   & 71.6          \\
                      & \cmark                                      & \xmark & 80.8  & 45.9   & 72.4~(+0.8)          \\
                      & \cmark                                      & \cmark & 82.7 & 52.5 & \textbf{75.5}~(+3.9) \\
      \bottomrule
    \end{tabular}
  
  \end{adjustbox}
  \vspace{-2mm}
\end{table}

==> a_tables/abl_lr.tex <==
\begin{table}[t]
  \centering
  \caption{
     Parameter search of hyper-parameter in flexible initial learning rate, $\lambda_{lr}$. All experiments are conducted on VOC 15-1.
    % SSUL-M denotes the result using exemplar memory.
  }
  \label{tab:abl_lr}
  \begin{adjustbox}{max width=\linewidth}
     \begin{tabular}{cc|ccc}
      \toprule
      \multirow{2}{*}{{Method}}  &\multirow{2}{*}{$\lambda_{lr}$} & \multicolumn{3}{c}{\textbf{VOC 15-1 (6 steps)}}                                                                  \\
                          &                                       & 0-15          & 16-20         & all                   \\ \midrule
       \multirow{5}{*}{CoinSeg}                             
                        & $10^{-4}$ & 83.0          & 48.4          & 74.5                  \\
                        & $10^{-3}$ & 82.7          & 52.5          & \textbf{75.5}          \\
                        & $0.01$ & 82.6          & 51.1          & 75.1          \\
                        & $0.1$ & 82.3 & 50.7 & 74.8 \\
                        & $1$ & 81.3 & 49.6 & 73.8 \\
      \bottomrule
    \end{tabular}
  
  \end{adjustbox}
  \vspace{-2mm}
\end{table}

==> a_tables/abl_lr_10-1.tex <==
\begin{table}[h]
  \centering

  \caption{
    More detailed hyperparameter search of $\lambda_{lr}$ on VOC 10-1, within similar magnitudes.
  }
  \label{tab:abl_lr10-1}
  \begin{adjustbox}{max width=\linewidth}
     \begin{tabular}{cc|ccc}
      \toprule
      \multirow{2}{*}{{Method}}  &\multirow{2}{*}{$\lambda_{lr}$} & \multicolumn{3}{c}{\textbf{VOC 10-1 (11 steps)}}                                                                  \\
                          &                                       & 0-10          & 11-20         & all                   \\ \midrule
       \multirow{3}{*}{CoinSeg}       
                        & $1 \times 10^{-4}$ & 80.4         & 58.6          &   69.9                \\
                        & $5 \times 10^{-4}$ & 80.2         & 59.1          &   70.2                \\
                        & $1\times10^{-3}$ & 80.1          & 60.0          & \textbf{70.5}          \\
                        & $2\times 10^{-3}$ & 79.8          & 59.5          &   70.1        \\
                        & $5\times 10^{-3}$ & 79.0          & 59.2          &   69.6        \\

      \bottomrule
    \end{tabular}
  
  \end{adjustbox}

\end{table}

==> a_tables/abl_reg.tex <==
\begin{table}[t]
  \centering
  \caption{
     Parameter search of hyper-parameter of regularization constraints, $\lambda_r$. All experiments are conducted on VOC 15-1.
    % SSUL-M denotes the result using exemplar memory.
  }
  \label{tab:abl_reg}
  \begin{adjustbox}{max width=\linewidth}
     \begin{tabular}{cc|ccc}
      \toprule
      \multirow{2}{*}{{Method}}  &\multirow{2}{*}{$\lambda_r$} & \multicolumn{3}{c}{\textbf{VOC 15-1 (6 steps)}}                                                                  \\
                          &                                       & 0-15          & 16-20         & all                   \\ \midrule
       \multirow{5}{*}{CoinSeg}                             
                                & $10^{-3}$ & 80.9          & 53.3          & 74.3                 \\
                                & $0.01$ &  81.9         & 52.6          & 74.9          \\
                                & $0.1$ & 82.7          & 52.5          & \textbf{75.5}          \\
                                & $1$ & 81.7 & 50.6 & 74.3 \\
                                & $10$ & 80.8 & 50.4 & 73.5 \\
      \bottomrule
    \end{tabular}
  
  \end{adjustbox}
  \vspace{-2mm}
\end{table}

==> a_tables/abl_same_magnitude.tex <==
\begin{table}[h]
\color[rgb]{0,0,0.18} % 文字颜色
    \vspace{-2mm}
  \centering
  \caption{
     Hyperparameter search of $\lambda_c$ within a similar magnitude, in VOC 15-1.
  }
  \label{tab:sameMagnitude}
  \begin{adjustbox}{max width=0.96\linewidth}

    \begin{tabular}{c|ccc}
\toprule
\multirow{2}{*}{$\lambda_c$} & \multicolumn{3}{c}{VOC 15-1 (6 steps)} \\
 & 0-15 & 16-20 & all \\ \midrule
$0.75\times10^{-2}$ & 82.5 & 53.0 & 75.5(+0.0) \\
$1\times10^{-2}$ & 82.7 & 52.5 & \textbf{75.5} \\
$3\times10^{-2}$ & 82.7 & 52.3 & 75.4(-0.1) \\
$5\times10^{-2}$ & 82.6 & 51.4 & 75.1(-0.4) \\
$7\times10^{-2}$ & 82.6 & 52.0 & 75.2(-0.3) \\ \bottomrule
\end{tabular}
  
  \end{adjustbox}
  \vspace{-6mm}
\end{table}

==> a_tables/abl_tau.tex <==


\begin{table}[t]
  \centering
  \caption{
     Parameter search of hyper-parameter: threshold $\tau$ for pseudo-label. All experiments are conducted on VOC 15-1.
    % SSUL-M denotes the result using exemplar memory.
  }
  \label{tab:abl_tau}
  \begin{adjustbox}{max width=\linewidth}
     \begin{tabular}{cc|ccc}
      \toprule
      \multirow{2}{*}{{Method}}  &\multirow{2}{*}{$\tau$} & \multicolumn{3}{c}{\textbf{VOC 15-1 (6 steps)}}                                                                  \\
                          &                                       & 0-15          & 16-20         & all                   \\ \midrule
       \multirow{5}{*}{CoinSeg}                             & $0.1$ & 81.4          & 47.5          & 73.3                  \\
                                                            & $0.3$ &  81.3         & 49.7          & 73.8          \\
                                                            & $0.5$ & 82.0          & 50.6          & 74.5          \\
                                                            & $0.7$ & 82.7          & 52.5          & \textbf{75.5} \\
                                                            & $0.9$ & 81.1 & 51.9 & 74.1 \\
      \bottomrule
    \end{tabular}
  
  \end{adjustbox}
  \vspace{-2mm}
\end{table}

==> a_tables/compareofbackbone.tex <==
\begin{table*}[t]
  \centering
  \caption{
     Comparisons of CoinSeg with different backbones.  \dag: Re-implemented with Swin-B backbone.
  }
  \label{tab:cmpofbkbn}
  \begin{adjustbox}{max width=0.9\linewidth}
     \begin{tabular}{l|c|ccc|ccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multicolumn{3}{c|}{\textbf{VOC 10-1 (11 steps)}} & \multicolumn{3}{c|}{\textbf{VOC 15-1 (6 steps)}} & \multicolumn{3}{c|}{\textbf{VOC 19-1 (2 steps)}} & \multicolumn{3}{c|}{\textbf{VOC 15-5 (2 steps)}} & \multicolumn{3}{c}{\textbf{VOC 2-2 (10 steps)}} \\
 &  & 0-10 & 11-20 & all & 0-15 & 16-20 & all & 0-19 & 20 & all & 0-15 & 16-20 & all & 0-2 & 3-20 & all \\ \midrule

\methodname & Resnet101 & 73.7 & 45.0 & 60.1 & 80.6 & 36.2 & 70.1 & 80.7 & 29.4 & 78.3 & 80.8 & 31.0 & 68.9 & 68.3 & 46.2 & 49.4 \\
CoinSeg\dag & Swin-B & 80.0 & 63.4 & 72.5 & 82.7 & 52.5 & 75.5 & 81.5 & 44.8 & 79.8 & 82.1 & 63.2 & 77.6 & 70.1 & 63.3 & 64.3 \\  
\bottomrule
\end{tabular}
  
  \end{adjustbox}
  \vspace{-2mm}
\end{table*}

==> a_tables/disjoint.tex <==
\begin{table*}[!htp]
\centering
\caption{
    Experimental results on Pascal VOC 2012 for \textit{disjoint} setup. \dag: CoinSeg with Swin-B backbone.
    % SSUL-M denotes the result using exemplar memory.
  }
  
  \begin{adjustbox}{max width=\linewidth}
\begin{tabular}{l|ccc|ccc|ccc} 
\toprule
\multirow{2}{*}{Method}                  & \multicolumn{3}{c|}{\textbf{VOC 15-1 (6 steps)}} & \multicolumn{3}{c|}{\textbf{VOC 19-1 (2 steps)}} & \multicolumn{3}{c}{\textbf{VOC 15-5 (2 steps)}}  \\
            & 0-15  & 16-20 & all                              & 0-19  & 20    & all                              & 0-15  & 16-20 & all                              \\ 
\midrule

LwF-MC~\cite{LwF_li2017learning}            & 4.5  & 7.0  & 5.2                             & 63.0 & 13.2 & 60.5                            & 67.2 & 41.2 & 60.7                            \\
ILT~\cite{ILT_michieli2019incremental}               & 3.7  & 5.7  & 4.2                             & 69.1 & 16.4 & 66.4                            & 63.2 & 39.5 & 57.3                            \\
MiB~\cite{MiB}               & 46.2 & 12.9 & 37.9                            & 69.6 & 25.6 & 67.4                            & 71.8 & 43.3 & 64.7                            \\
SDR~\cite{SDR} & 59.4 & 14.3 & 48.7 & 70.8 & 31.4 & 68.9 & 74.6 & 44.1 & 67.3 \\
PLOP~\cite{PLOP}              & 57.9 & 13.7 & 46.5                            & 75.4 & 38.9 & 73.6                            & 71.0 & 42.8 & 64.3                            \\
RCIL~\cite{SDR} & 66.1 & 18.2 & 54.7 & 68.9 & 15.0 & 66.3 & 75.0 & 42.8 & 67.3 \\
SSUL~\cite{SSUL}              & 74.0 & 32.2 & 64.0                            & 77.4 & 22.4 & 74.8                            & 76.4 & 45.6 & 69.1                            \\
SSUL-M~\cite{SSUL}            & 76.5 & 43.4 & 68.6                            & 77.6 & 43.9 & 76.0                            & 76.5 & 48.6 & 69.8                            \\ 

MicroSeg~\cite{MicroSeg}   & 73.7 & 24.1 & 61.9                            & 80.6 & 16.0 & 77.4                          & 77.4 & 43.4 & 69.3                            \\
MicroSeg-M~\cite{MicroSeg} & 80.0  & 47.6  & 72.3                            & 81.1  & 45.1  & 79.4                             & 80.7  & 55.2  & 74.7                             \\ 
CoinSeg~(Ours)   & 75.6 & 30.9 & 64.9                            & 80.5 & 25.1 & 77.9                    & 79.6 & 43.8 & 71.1                            \\
CoinSeg-M~(Ours) & 80.9  & 47.4  & 72.9                            & 80.8  & 50.6  & 79.4                             & 81.7 & 58.9  & 76.3                             \\ 
\midrule
CoinSeg\dag~(Ours)   & \textbf{82.0} & 46.1 & 73.4                            & 82.0 & 34.0 & 80.2                          & 82.1 & 55.3 & 75.7                            \\
CoinSeg-M\dag~(Ours) & \textbf{82.0}  & \textbf{49.6}  & \textbf{74.3}                             & \textbf{82.6}  & \textbf{66.3}  & \textbf{81.8}                             & \textbf{82.9} & \textbf{61.7}  & \textbf{77.9}                             \\ 
\bottomrule
\end{tabular}
  \end{adjustbox}
  \label{tab:disjoint_all}
\end{table*}



==> a_tables/resnet.tex <==
\begin{table*}[t!]
  \centering
\caption{
    Comparison with state-of-the-art methods on Pascal VOC 2012 with ResNet101. \textcolor{lightgray}{Joint} is the upperbound.
  }
  \label{tab:resnet}
  \begin{adjustbox}{max width=\linewidth}
  \begin{tabular}{l|c|ccc|ccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multicolumn{3}{c|}{\textbf{VOC 10-1 (11 steps)}} & \multicolumn{3}{c|}{\textbf{VOC 15-1 (6 steps)}} & \multicolumn{3}{c|}{\textbf{VOC 19-1 (2 steps)}} & \multicolumn{3}{c|}{\textbf{VOC 15-5 (2 steps)}} & \multicolumn{3}{c}{\textbf{VOC 2-2 (10 steps)}} \\
 &  & 0-10 & 11-20 & all & 0-15 & 16-20 & all & 0-19 & 20 & all & 0-15 & 16-20 & all & 0-2 & 3-20 & all \\ \midrule
\textcolor{lightgray}{Joint} & \textcolor{lightgray}{ResNet101} & \textcolor{lightgray}{82.1}  & \textcolor{lightgray}{79.6} & \textcolor{lightgray}{80.9} & \textcolor{lightgray}{82.7} & \textcolor{lightgray}{75.0} & \textcolor{lightgray}{80.9} & \textcolor{lightgray}{81.0} & \textcolor{lightgray}{79.1} & \textcolor{lightgray}{80.9} & \textcolor{lightgray}{82.7} & \textcolor{lightgray}{75.0} & \textcolor{lightgray}{80.9} & \textcolor{lightgray}{76.5} & \textcolor{lightgray}{81.6} & \textcolor{lightgray}{80.9} \\
LwF-MC~\cite{LwF_li2017learning} & ResNet101 & 4.7 & 5.9 & 4.9 & 6.4 & 8.4 & 6.9 & 64.4 & 13.3 & 61.9 & 58.1 & 35.0 & 52.3 & 3.5 & 4.7 & 4.5\\
ILT~\cite{ILT_michieli2019incremental} & ResNet101 & 7.2 & 3.7 & 5.5 & 8.8 & 8.0 & 8.6 & 67.8 & 10.9 & 65.1 & 67.1 & 39.2 & 60.5 & 5.8 & 5.0 & 5.1 \\
MiB~\cite{MiB} & ResNet101 & 12.3 & 13.1 & 12.7 & 34.2 & 13.5 & 29.3 & 71.4 & 23.6 & 69.2 & 76.4 & 50.0 & 70.1 & 41.1 & 23.4 & 25.9 \\
SDR~\cite{SDR} & ResNet101 & 32.1 & 17.0 & 24.9 & 44.7 & 21.8 & 39.2 & 69.1 & 32.6 & 67.4 & 57.4 & 52.6 & 69.9 & 13.0 & 5.1 & 6.2 \\
PLOP~\cite{PLOP} & ResNet101 & 44.0 & 15.5 & 30.5 & 65.1 & 21.1 & 54.6 & 75.4 & 37.4 & 73.5 & 75.7 & 51.7 & 70.1 & 24.1 & 11.9 & 13.7 \\
RCIL~\cite{RCIL} & ResNet101 & 55.4 & 15.1 & 34.3 & 70.6 & 23.7 & 59.4 & 68.5 & 12.1 & 65.8 & 78.8 & 52.0 & 72.4 & 28.3 & 19.0 & 19.4 \\
SSUL~\cite{SSUL} & ResNet101 & 71.3 & 46.0 & 59.3 & 77.3 & 36.6 & 67.6 & 77.7 & 29.7 & 75.4 & 77.8 & 50.1 & 71.2 & 62.4 & 42.5 & 45.3 \\
SSUL-M\cite{SSUL} & ResNet101 & 74.0 & 53.2 & 64.1 & 78.4 & 49.0 & 71.4 & 77.8 & 49.8 & 76.5 & 78.4 & 55.8 & 73.0 & 58.8 & 45.8 & 47.6 \\
MicroSeg~\cite{MicroSeg} & ResNet101 & 72.6 & 48.7 & 61.2 & 80.1 & 36.8 & 69.8 & 78.8 & 14.0 & 75.7 & 80.4 & 52.8 & 73.8 & 61.4 & 40.6 & 43.5 \\
MicroSeg-M~\cite{MicroSeg} & ResNet101 & \textbf{77.2} & 57.2 & \textbf{67.7} & 81.3 & 52.5 & 74.4 & 79.3 & 62.9 & 78.5 & \textbf{82.0} & 59.2 & \textbf{76.6} & 60.0 & 50.9 & 52.2 \\ 
\midrule
CoinSeg~(Ours) & ResNet101 & 73.7 & 45.0 & 60.1 & 80.6 & 36.2 & 70.1 & \textbf{80.7} & 29.4 & 78.3 & 80.8 & 31.0 & 68.9 & 68.3 & 46.2 & 49.4 \\
CoinSeg-M~(Ours) & ResNet101 & 71.1 & \textbf{60.2} & 65.9 & \textbf{81.5} & \textbf{54.0} & \textbf{75.0} & 80.3 & \textbf{44.8} & \textbf{78.6} & 81.3 & \textbf{61.3} & \textbf{76.6} & \textbf{66.7} & \textbf{53.9} & \textbf{55.7} \\


\bottomrule
\end{tabular}
  \end{adjustbox}
\end{table*}





==> a_tables/vocwithclass.tex <==


%------------------------------------------------------------------------------------
\begin{table*}[h]
  \centering
  \caption{Detailed experimental results of CoinSeg over each class.}
  \begin{adjustbox}{max width=\linewidth}
\begin{tabular}{c|ccccccccccc}
\toprule
\multirow{4}{*}{\textbf{VOC 10-1}} & bg & aero & bike & bird & boat & bottle & bus & car & cat & chair & cow \\ \cline{2-12} 
 & 88.0 & 89.9 & 40.8 & 94.1 & 76.3 & 88.5 & 91.1 & 89.7 & 96.2 & 48.4 & 77.2 \\ 
 \cline{2-12} 
 &  {table} &  {dog} &  {horse} &  {mbike} &  {person} &  {plant} &  {sheep} &  {sofa} &  {train} & \multicolumn{1}{c}{TV} &  {\textbf{mIoU}} \\ \cline{2-12} 
 & 37.8 & 89.4 & 75.3 & 83.7 & 85.5 & 47.1 & 59.5 & 27.4 & 74.8 & 53.2 & \textbf{72.5}  \\ 
 \midrule
\multirow{4}{*}{\textbf{VOC 15-1}} & bg & aero & bike & bird & boat & bottle & bus & car & cat & chair & cow \\ \cline{2-12} 
 & 90.3 & 89.8 & 43.5 & 95.2 & 79.3 & 88.0 & 91.2 & 90.8 & 96.3 & 47.1 & 78.1 \\ \cline{2-12} 
 &  {table} &  {dog} &  {horse} &  {mbike} &  {person} &  {plant} &  {sheep} &  {sofa} &  {train} & \multicolumn{1}{c}{TV} &  {\textbf{mIoU}} \\ \cline{2-12} 
 & 68.5 & 93.3 & 91.0 & 92.0 & 89.7 & 43.7 & 64.1 & 27.0 & 72.7 & 55.4 & \textbf{75.5} \\ 
 \midrule
\multirow{4}{*}{\textbf{VOC 19-1}} & bg & aero & bike & bird & boat & bottle & bus & car & cat & chair & cow \\ \cline{2-12} 
 & 93.9  & 91.8  & 43.0 & 94.5 & 76.4 & 87.2 & 95.0 & 89.6 & 96.5 & 49.1 & 91.5 \\ 
 \cline{2-12} 
 &  {table} &  {dog} &  {horse} &  {mbike} &  {person} &  {plant} &  {sheep} &  {sofa} &  {train} & \multicolumn{1}{c}{TV} &  {\textbf{mIoU}} \\ \cline{2-12} 
 & 65.9 & 89.7 & 90.1 & 90.3 & 90.9 & 63.0 & 93.0 & 54.0 & 86.0 & 44.8 & \textbf{79.8} \\ 
 \midrule
\multirow{4}{*}{\textbf{VOC 15-5}} & bg & aero & bike & bird & boat & bottle & bus & car & cat & chair & cow \\ \cline{2-12} 
 & 91.3 & 90.9 & 43.8 & 95.4 & 74.5 & 85.2 & 90.0 & 91.3 & 95.2 & 49.1 & 79.5 \\ \cline{2-12} 
 &  {table} &  {dog} &  {horse} &  {mbike} &  {person} &  {plant} &  {sheep} &  {sofa} &  {train} & \multicolumn{1}{c}{TV} &  {\textbf{mIoU}} \\ \cline{2-12} 
 & 66.7 & 90.5 & 91.0 & 90.9 & 90.1 & 55.2 & 72.4 & 31.3 & 84.0 & 73.1 & \textbf{77.6} \\ 
 \midrule
 % 2-2
\multicolumn{1}{c|}{\multirow{4}{*}{\textbf{VOC 2-2}}} & bg & aero & bike & bird & boat & bottle & bus & car & cat & chair & cow \\ \cline{2-12} 
\multicolumn{1}{l|}{} & 89.1 & 85.4 & 35.8 & 53.2 & 56.9 & 76.7 & 88.5 & 80.3 & 88.0 & 18.3 & 64.4 \\ \cline{2-12} 
\multicolumn{1}{l|}{} &  {table} &  {dog} &  {horse} &  {mbike} &  {person} &  {plant} &  {sheep} &  {sofa} &  {train} & \multicolumn{1}{c}{TV} &  {\textbf{mIoU}} \\ \cline{2-12} 
\multicolumn{1}{l|}{} & 43.0 & 59.2 & 64.9 & 79.8 & 80.8 & 60.2 & 51.8 & 32.4 & 74.1 & 67.9 & \textbf{64.3} \\ 
\bottomrule
\end{tabular}
  \end{adjustbox}
  \label{tab:voc_class}
\end{table*}

==> tables/ablation.tex <==

\begin{table}[t]
  \centering
  \caption{
     Ablation Studies for our proposed methods. FT: flexible tuning; \textit{Coin}: contrast inter- and intra-class representations.
  }
  \label{tab:ablation}
  \begin{adjustbox}{max width=\linewidth}
     \begin{tabular}{ccc|ccc}
      \toprule
      \multirow{2}{*}{{Backbone}} & parameter &\multirow{2}{*}{\textit{Coin}} & \multicolumn{3}{c}{\textbf{VOC 15-1 (6 steps)}}                                                                  \\
                          & strategy                                    &  & 0-15          & 16-20         & all                   \\ \midrule
      Resnet101                & Freeze                                      & \xmark & 74.9          & 26.4          & 63.3                  \\
      Swin-B                & Freeze                                      & \xmark & 79.5          & 42.4          & 70.5~(+7.2)          \\
      Swin-B                & FT                                      & \xmark & 80.4          & 43.7          & 71.6~(+8.3)          \\
      Swin-B                & FT                                      & \cmark & 82.7 & 52.5 & \textbf{75.5}~(+12.2) \\
      \bottomrule
    \end{tabular}
  
  \end{adjustbox}
  \vspace{-2mm}
\end{table}
